Robust Semi-Supervised Anomaly Detection via Adversarially Learned Continuous Noise Corruption

Anomaly detection is the task of recognising novel samples which deviate significantly from pre-establishednormality. Abnormal classes are not present during training meaning that models must learn effective rep-resentations solely across normal class data samples. Deep Autoencoders (AE) have been widely used foranomaly detection tasks, but suffer from overfitting to a null identity function. To address this problem, weimplement a training scheme applied to a Denoising Autoencoder (DAE) which introduces an efficient methodof producing Adversarially Learned Continuous Noise (ALCN) to maximally globally corrupt the input priorto denoising. Prior methods have applied similar approaches of adversarial training to increase the robustnessof DAE, however they exhibit limitations such as slow inference speed reducing their real-world applicabilityor producing generalised obfuscation which is more trivial to denoise. We show through rigorous evaluationthat our ALCN method of regularisation during training improves AUC performance during inference whileremaining efficient over both classical, leave-one-out novelty detection tasks with the variations-: 9 (normal)vs. 1 (abnormal) & 1 (normal) vs. 9 (abnormal); MNIST - AUCavg: 0.890 & 0.989, CIFAR-10 - AUCavg: 0.670& 0.742, in addition to challenging real-world anomaly detection tasks: industrial inspection (MVTEC-AD -AUCavg: 0.780) and plant disease detection (Plant Village - AUC: 0.770) when compared to prior approaches.

==> figures/ComparisonDiagram.tex <==
 \begin{figure*}[htb!]
\centering
\includegraphics[width=\linewidth]{img/ComparisonDiagram2.pdf}
\vspace{-0.8cm}
\caption{Comparison between prior methods (A \cite{Kingma2013}, B \cite{bengio2013generalized}) and ours (C).}
\label{fig:comparison}
\end{figure*}



==> tables/MNISTCIFER2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}


\begin{table*}[htb!]

\centering
\caption{Quantitative results (class name indicates AUROC, $AUC_{avg}$ of all classes) of models across MNIST \cite{lecun-mnisthandwrittendigit-2010} (upper) and CIFAR-10 \cite{Krizhevsky09learningmultiple} (lower) datasets.}
\resizebox{500pt}{!}{
\begin{tabular}{|l|lllllllllll|}
\hline
\multirow{2}{*}{{\bf Model}} &
  \multicolumn{11}{c|}{\textbf{MNIST \cite{lecun-mnisthandwrittendigit-2010}}} \\ \cline{2-12}
 &
  \multicolumn{1}{l|}{\textbf{0}} &
  \multicolumn{1}{l|}{\textbf{1}} &
  \multicolumn{1}{l|}{\textbf{2}} &
  \multicolumn{1}{l|}{\textbf{3}} &
  \multicolumn{1}{l|}{\textbf{4}} &
  \multicolumn{1}{l|}{\textbf{5}} &
  \multicolumn{1}{l|}{\textbf{6}} &
  \multicolumn{1}{l|}{\textbf{7}} &
  \multicolumn{1}{l|}{\textbf{8}} &
  \multicolumn{1}{l|}{\textbf{9}} &
  \textbf{$AUC_{avg}$} \\ \hline \hline
  VAE \cite{Kingma2013} & 
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.10} &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{0.25} &
  \multicolumn{1}{l|}{0.35} &
  \multicolumn{1}{l|}{0.30} &
  \multicolumn{1}{l|}{0.43} &
  \multicolumn{1}{l|}{0.18} &
  \multicolumn{1}{l|}{0.50} &
  \multicolumn{1}{l|}{0.10} &
  0.34 \\ \hline
AnoGAN \cite{Schlegl2017} &
  \multicolumn{1}{l|}{0.61} &
  \multicolumn{1}{l|}{0.30} &
  \multicolumn{1}{l|}{0.54} &
  \multicolumn{1}{l|}{0.44} &
  \multicolumn{1}{l|}{0.43} &
  \multicolumn{1}{l|}{0.42} &
  \multicolumn{1}{l|}{0.48} &
  \multicolumn{1}{l|}{0.36} &
  \multicolumn{1}{l|}{0.40} &
  \multicolumn{1}{l|}{0.34} &
  0.43 \\ \hline
EGBAD \cite{zenati2018} &
  \multicolumn{1}{l|}{0.78} &
  \multicolumn{1}{l|}{0.29} &
  \multicolumn{1}{l|}{0.67} &
  \multicolumn{1}{l|}{0.52} &
  \multicolumn{1}{l|}{0.45} &
  \multicolumn{1}{l|}{0.43} &
  \multicolumn{1}{l|}{0.57} &
  \multicolumn{1}{l|}{0.40} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.35} &
  0.50 \\ \hline
GANomaly \cite{Akcay2018} &
  \multicolumn{1}{l|}{0.89} &
  \multicolumn{1}{l|}{0.65} &
  \multicolumn{1}{l|}{0.93} &
  \multicolumn{1}{l|}{0.80} &
  \multicolumn{1}{l|}{0.82} &
  \multicolumn{1}{l|}{0.85} &
  \multicolumn{1}{l|}{0.84} &
  \multicolumn{1}{l|}{0.69} &
  \multicolumn{1}{l|}{0.87} &
  \multicolumn{1}{l|}{0.55} &
  0.79 \\ \hline
  
DAE &
  \multicolumn{1}{l|}{0.84} &
  \multicolumn{1}{l|}{0.97} &
  \multicolumn{1}{l|}{0.79} &
  \multicolumn{1}{l|}{0.64} &
  \multicolumn{1}{l|}{0.53} &
  \multicolumn{1}{l|}{0.61} &
  \multicolumn{1}{l|}{0.66} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.71} &
  \multicolumn{1}{l|}{0.57} &
  0.69 \\ \hline
DAE+Random Noise &
  \multicolumn{1}{l|}{0.84} &
  \multicolumn{1}{l|}{0.93} &
  \multicolumn{1}{l|}{0.66} &
  \multicolumn{1}{l|}{0.66} &
  \multicolumn{1}{l|}{0.52} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{0.72} &
  \multicolumn{1}{l|}{0.56} &
  \multicolumn{1}{l|}{0.75} &
  \multicolumn{1}{l|}{0.53} &
  0.68 \\ \hline
\begin{tabular}[c]{@{}l@{}}DAE+Gaussian Noise\\ $\sim N(0, 0.5)$ \end{tabular} &
  \multicolumn{1}{l|}{0.88} &
  \multicolumn{1}{l|}{0.97} &
  \multicolumn{1}{l|}{0.77} &
  \multicolumn{1}{l|}{0.66} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{0.75} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.71} &
  \multicolumn{1}{l|}{0.57} &
  0.70 \\ \hline
DAE+Adversarial Noise &
  \multicolumn{1}{l|}{\textbf{0.97}} &
  \multicolumn{1}{l|}{\textbf{0.97}} &
  \multicolumn{1}{l|}{\textbf{0.96}} &
  \multicolumn{1}{l|}{\textbf{0.89}} &
  \multicolumn{1}{l|}{\textbf{0.85}} &
  \multicolumn{1}{l|}{\textbf{0.88}} &
  \multicolumn{1}{l|}{\textbf{0.92}} &
  \multicolumn{1}{l|}{\textbf{0.80}} &
  \multicolumn{1}{l|}{\textbf{0.93}} &
  \multicolumn{1}{l|}{\textbf{0.76}} &
  \textbf{0.89} \\ \hline \hline 
 
 \multirow{2}{*}{{\bf Model}} & \multicolumn{11}{c|}{\textbf{CIFAR-10 \cite{Krizhevsky09learningmultiple}}} \\ \cline{2-12}

& \multicolumn{1}{l|}{\textbf{Airplane}} &
  \multicolumn{1}{l|}{\textbf{Automobile}} &
  \multicolumn{1}{l|}{\textbf{Bird}} &
  \multicolumn{1}{l|}{\textbf{Cat}} &
  \multicolumn{1}{l|}{\textbf{Deer}} &
  \multicolumn{1}{l|}{\textbf{Dog}} &
  \multicolumn{1}{l|}{\textbf{Frog}} &
  \multicolumn{1}{l|}{\textbf{Horse}} &
  \multicolumn{1}{l|}{\textbf{Ship}} &
  \multicolumn{1}{l|}{\textbf{Truck}} &
  \textbf{$AUC_{avg}$} \\ \hline \hline
VAE \cite{Kingma2013} &
  \multicolumn{1}{l|}{0.59} &
  \multicolumn{1}{l|}{0.40} &
  \multicolumn{1}{l|}{0.52} &
  \multicolumn{1}{l|}{0.44} &
  \multicolumn{1}{l|}{0.46} &
  \multicolumn{1}{l|}{0.50} &
  \multicolumn{1}{l|}{0.38} &
  \multicolumn{1}{l|}{0.51} &
  \multicolumn{1}{l|}{0.64} &
  \multicolumn{1}{l|}{0.49} &
  0.49 \\ \hline
AnoGAN \cite{Schlegl2017} &
  \multicolumn{1}{l|}{0.51} &
  \multicolumn{1}{l|}{0.49} &
  \multicolumn{1}{l|}{0.41} &
  \multicolumn{1}{l|}{0.40} &
  \multicolumn{1}{l|}{0.34} &
  \multicolumn{1}{l|}{0.39} &
  \multicolumn{1}{l|}{0.34} &
  \multicolumn{1}{l|}{0.41} &
  \multicolumn{1}{l|}{0.56} &
  \multicolumn{1}{l|}{0.51} &
  0.44 \\ \hline
EGBAD \cite{zenati2018} &
  \multicolumn{1}{l|}{0.58} &
  \multicolumn{1}{l|}{0.52} &
  \multicolumn{1}{l|}{0.39} &
  \multicolumn{1}{l|}{0.45} &
  \multicolumn{1}{l|}{0.37} &
  \multicolumn{1}{l|}{0.49} &
  \multicolumn{1}{l|}{0.36} &
  \multicolumn{1}{l|}{0.54} &
  \multicolumn{1}{l|}{0.42} &
  \multicolumn{1}{l|}{0.55} &
  0.47 \\ \hline
GANomaly \cite{Akcay2018} &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{0.51} &
  \multicolumn{1}{l|}{\textbf{0.58}} &
  \multicolumn{1}{l|}{0.59} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{0.68} &
  \multicolumn{1}{l|}{\textbf{0.61}} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{0.62} &
  0.61 \\ \hline
DAE &
  \multicolumn{1}{l|}{0.50} &
  \multicolumn{1}{l|}{0.68} &
  \multicolumn{1}{l|}{0.61} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.69} &
  \multicolumn{1}{l|}{0.53} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{0.60} &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{\textbf{0.71}} &
  0.61 \\ \hline
DAE+Random Noise &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{0.53} &
  \multicolumn{1}{l|}{0.54} &
  \multicolumn{1}{l|}{0.54} &
  \multicolumn{1}{l|}{0.65} &
  \multicolumn{1}{l|}{0.59} &
  \multicolumn{1}{l|}{0.64} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.66} &
  \multicolumn{1}{l|}{0.63} &
  0.60 \\ \hline
\begin{tabular}[c]{@{}l@{}}DAE+Gaussian Noise\\ $\sim N(0, 0.5)$\end{tabular} &
  \multicolumn{1}{l|}{0.57} &
  \multicolumn{1}{l|}{0.68} &
  \multicolumn{1}{l|}{0.57} &
  \multicolumn{1}{l|}{0.54} &
  \multicolumn{1}{l|}{0.65} &
  \multicolumn{1}{l|}{0.54} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.52} &
  \multicolumn{1}{l|}{0.57} &
  \multicolumn{1}{l|}{0.53} &
  0.57 \\ \hline
DAE+Adversarial Noise &
  \multicolumn{1}{l|}{\textbf{0.77}} &
  \multicolumn{1}{l|}{\textbf{0.71}} &
  \multicolumn{1}{l|}{\textbf{0.62}} &
  \multicolumn{1}{l|}{0.57} &
  \multicolumn{1}{l|}{\textbf{0.72}} &
  \multicolumn{1}{l|}{\textbf{0.62}} &
  \multicolumn{1}{l|}{\textbf{0.72}} &
  \multicolumn{1}{l|}{0.60} &
  \multicolumn{1}{l|}{\textbf{0.66}} &
  \multicolumn{1}{l|}{0.69} &
  \textbf{0.67} \\ \hline
\end{tabular}
}
% \caption{Quantitative results of models across MNIST (upper) and CIFAR-10 (lower) using Area Under Receiver Operator Characteristics (AUROC) metric.}
\label{tab:MNISTCIFAR}
% \label{tab:map}
\end{table*}

==> tables/MVTEC2.tex <==
\begin{table*}[htb!]

\centering
\caption{Quantitative results (class name indicates AUROC, $AUC_{avg}$ of all classes) of models MVTEC-AD \cite{bergmann2019mvtec} dataset.}


\resizebox{500pt}{!}{
\begin{tabular}{|l|llllllllllllllll|}
\hline
\label{tab:MVTEC}
\multirow{2}{*}{\textbf{Model}} &
  \multicolumn{16}{c|}{\textbf{MVTEC-AD \cite{bergmann2019mvtec}}} \\ \cline{2-17} 
 &
  \multicolumn{1}{c|}{\textbf{Bottle}} &
  \multicolumn{1}{c|}{\textbf{Cable}} &
  \multicolumn{1}{c|}{\textbf{Capsule}} &
  \multicolumn{1}{c|}{\textbf{Carpet}} &
  \multicolumn{1}{c|}{\textbf{Grid}} &
  \multicolumn{1}{c|}{\textbf{Hazelnut}} &
  \multicolumn{1}{c|}{\textbf{Leather}} &
  \multicolumn{1}{c|}{\textbf{Metal Nut}} &
  \multicolumn{1}{c|}{\textbf{Pill}} &
  \multicolumn{1}{c|}{\textbf{Screw}} &
  \multicolumn{1}{c|}{\textbf{Tile}} &
  \multicolumn{1}{c|}{\textbf{Toothbrush}} &
  \multicolumn{1}{c|}{\textbf{Transistor}} &
  \multicolumn{1}{c|}{\textbf{Wood}} &
  \multicolumn{1}{c|}{\textbf{Zipper}} &
  \multicolumn{1}{c|}{\textbf{$AUC_{avg}$}} \\ \hline \hline
  
  VAE \cite{Kingma2013} &
  \multicolumn{1}{l|}{0.66} &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{0.61} &
  \multicolumn{1}{l|}{0.51} &
  \multicolumn{1}{l|}{0.52} &
  \multicolumn{1}{l|}{0.30} &
  \multicolumn{1}{l|}{0.41} &
  \multicolumn{1}{l|}{0.66} &
  \multicolumn{1}{l|}{0.51} &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{0.21} &
  \multicolumn{1}{l|}{0.30} &
  \multicolumn{1}{l|}{0.65} &
  \multicolumn{1}{l|}{0.87} &
  \multicolumn{1}{l|}{\textbf{0.87}} &
  0.58 \\ \hline
  
\rowcolor{blue!5}
AnoGAN \cite{Schlegl2017} &
  \multicolumn{1}{l|}{0.80} &
  \multicolumn{1}{l|}{0.48} &
  \multicolumn{1}{l|}{0.44} &
  \multicolumn{1}{l|}{0.34} &
  \multicolumn{1}{l|}{\textbf{0.87}} &
  \multicolumn{1}{l|}{0.26} &
  \multicolumn{1}{l|}{0.45} &
  \multicolumn{1}{l|}{0.28} &
  \multicolumn{1}{l|}{0.71} &
  \multicolumn{1}{l|}{1} &
  \multicolumn{1}{l|}{0.40} &
  \multicolumn{1}{l|}{0.44} &
  \multicolumn{1}{l|}{0.69} &
  \multicolumn{1}{l|}{0.57} &
  \multicolumn{1}{l|}{0.72} &
  0.56 \\ \hline
EGBAD \cite{zenati2018} &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{0.68} &
  \multicolumn{1}{l|}{0.52} &
  \multicolumn{1}{l|}{0.52} &
  \multicolumn{1}{l|}{0.54} &
  \multicolumn{1}{l|}{0.43} &
  \multicolumn{1}{l|}{0.55} &
  \multicolumn{1}{l|}{0.47} &
  \multicolumn{1}{l|}{0.57} &
  \multicolumn{1}{l|}{0.43} &
  \multicolumn{1}{l|}{0.79} &
  \multicolumn{1}{l|}{0.64} &
  \multicolumn{1}{l|}{0.73} &
  \multicolumn{1}{l|}{0.91} &
  \multicolumn{1}{l|}{0.58} &
  0.60 \\ \hline
\rowcolor{blue!5}
GANomaly \cite{Akcay2018} &
  \multicolumn{1}{l|}{0.89} &
  \multicolumn{1}{l|}{0.76} &
  \multicolumn{1}{l|}{0.73} &
  \multicolumn{1}{l|}{0.70} &
  \multicolumn{1}{l|}{0.71} &
  \multicolumn{1}{l|}{\textbf{0.79}} &
  \multicolumn{1}{l|}{\textbf{0.84}} &
  \multicolumn{1}{l|}{0.70} &
  \multicolumn{1}{l|}{0.74} &
  \multicolumn{1}{l|}{0.75} &
  \multicolumn{1}{l|}{0.79} &
  \multicolumn{1}{l|}{0.65} &
  \multicolumn{1}{l|}{\textbf{0.79}} &
  \multicolumn{1}{l|}{0.83} &
  \multicolumn{1}{l|}{0.75} &
  0.76 \\ \hline
\begin{tabular}[c]{@{}l@{}}$\text{DAE}_{256}$+\\ AdversarialNoise\end{tabular} &
  \multicolumn{1}{l|}{\textbf{0.94}} &
  \multicolumn{1}{l|}{\textbf{0.78}} &
  \multicolumn{1}{l|}{\textbf{0.86}} &
  \multicolumn{1}{l|}{\textbf{0.78}} &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{0.74} &
  \multicolumn{1}{l|}{0.62} &
  \multicolumn{1}{l|}{\textbf{0.86}} &
  \multicolumn{1}{l|}{\textbf{0.75}} &
  \multicolumn{1}{l|}{\textbf{1}} &
  \multicolumn{1}{l|}{\textbf{0.79}} &
  \multicolumn{1}{l|}{\textbf{0.65}} &
  \multicolumn{1}{l|}{0.73} &
  \multicolumn{1}{l|}{\textbf{0.93}} &
  \multicolumn{1}{l|}{0.70} &
  \textbf{0.78} \\ \hline
\end{tabular}
}

\end{table*}
